Shape and Reflectance Reconstruction in Uncontrolled Environments by Differentiable Rendering

Simultaneous reconstruction of geometry and reflectance properties in uncontrolled environments remains a challenging problem. In this paper, we propose an efficient method to reconstruct the scene's 3D geometry and reflectance from multi-view photography using conventional hand-held cameras. Our method automatically builds a virtual scene in a differentiable rendering system that roughly matches the real world's scene parameters, optimized by minimizing photometric objectives alternatingly and stochastically. With the optimal scene parameters evaluated, photo-realistic novel views for various viewing angles and distances can then be generated by our approach. We present the results of captured scenes with complex geometry and various reflection types. Our method also shows superior performance compared to state-of-the-art alternatives in novel view synthesis visually and quantitatively.

==> overview.tex <==
\section{Overview}
We illustrate our proposed framework in \figref{fig:tbd}: It takes a set of RGB images $I = \{I_k\}$ of the scene from arbitrary viewpoints and camera position as input. Then, our method automatically builds a virtual scene that roughly matches real world via parameter initialization, and iteratively optimize scene parameters for 3D geometry, diffuse and specular reflectance, camera pose and position, and environment lighting map by pushing the photometric consistency between rendering images and real photography in the same camera intrinsic and extrinsic. Finally, a set of optimized scene parameters can enable several photo-realistic applications: view synthesis, lighting editing, etc.
Mathematically, our system can be described as a function of desired parameters as, 
\begin{equation}\label{eqn:image_formation}
I = \Phi(\theta_{g}, \theta_{d}, \theta_{s}, \theta_{l}),
\end{equation} 
where $\Phi$ is the physically-based rendering process, which
simulates the light rays traveling in a virtual scene.  $\theta_{g} =
\{x_0, \dots, x_N\}$ is the set of 3D positions corresponding to the
mesh vertices.  $\theta_{d} = \{\theta_{d}(x_0), \dots,
\theta_{d}(x_N)\}$ is the set of diffuse per-vertex color
reflectance, with $\theta_{d}(x) \in \mathbb{R}^{3}$.  Similarly, $\theta_{s}$
is the set of specular reflectances.
The illumination in the scene is modeled as environmental lighting $l_0$,
approximated as a set of isotropic point sources $\theta_{l} = \{l_0, l_1, \dots, l_M\}$, $l_n$ is the intensity for $n$-th light sources.  
We use
Mitsuba2~\cite{NimierDavidVicini2019Mitsuba2} as our physically-based
rendering engine and renderer. Therefore,
it enables an iterative optimization pipeline that back propagates
rendering error to update scene parameters.
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.99\linewidth]{fig/pipeline2}
	\caption[]{Inverse parameter optimization pipeline.}
	\label{fig:tbd}
\end{figure} 


%\todo{Already mention here which SfM and MVS methods you use}
%We design our system in a manner of differentiable forward rendering and backward error propagation. 
%First, in the initialization step, 
%vertex diffuse reflectance $\theta_{d}$ by a differentiable rendering and back propagate error.  
%our method alternatively optimize scene parameters in \eqnref{eqn:image_formation}. 
%The example number of images can range from. We represent our image formation model for each taken image as a rendering function with unknown scene parameters, 
%This work presents a differentiable rendering and inverse reconstruction system for robust and efficient dense modeling from unordered images of real scene. 
%Given the multiple photographs from different viewpoints and captured distance, our system can jointly estimate 3D geometry and surface reflectance by minimizing pixelwise photometric objective in a manner of forward rendering and backward error propagation.
%\paragraph{Initial 3D Geometry and Reflectance Estimation} By given unordered images from multiple view points, we match feature points to generate sparse point cloud, and then apply MVS method to generate pixelwise dense matching to recover raw scene reflectance and 3D mesh.

%\paragraph{Multi-camera Parameters Estimation} For each view of the real scene, we recover camera positions and poses by utilizing SfM methods, and adjust camera parameters (fov, focal length, etc) to match the real cameras. 

%\paragraph{Lighting Condition Estimation}
%We set up one environment light source, and several diffuse directional light source.
%We set up several light source and optimize its position to simulate real world light

%\paragraph{Differentiable and Inverse Reconstruction}
%Given a initial guess of camera intrinsic and extrinsic, rough 3D mesh, we build a virtual scene that contains our 3D mesh object, virtual camera sensors that match real scene's camera position and pose, with a rough initial environment lighting map (e.g., constant white ambient light) in Mitsuba2.
%%We build a virtual scene with an estimated rough 3D geometry and reflectance with virtual sensors that matches real scene's camera position and pose, then with an initial environment lighting map in Mitsuba2. 
%We render image for each virtual camera sensors in Mitsuba2, and then minimize our objective by pushing virtual rendering images to be as similar as real camera observations with proper regularization. Rendering error then back propagates to update scene parameters for 3D geometry, diffuse and specular reflectance, environment lighting map by auto-diff mechanism and automatically gradient estimation for non-differentiable parameters. 
%Specifically, we start from initial estimated 3D mesh with vertex reflectance, our method optimize diffuse reflectance $\theta_{d}$ (sec 5), and optimize 3D geometry $\theta_{g}$ (sec 6) relying on $\theta_{d}$.
%After obtaining $\theta_{d}$ and $\theta_{g}$, our method update the camera position and pose $\theta_{c}$ and environment light map $\theta_{l}$ by pushing photometric consistency, which allow us further update specular reflection parameter $\theta_{s}$.
%We repeat this iterative optimization of inverse rendering and geometric reconstruction until the error
%converges.

Initialized by rough parameters for camera intrinsic and extrinsic and a coarse 3D mesh from MVS, we build a virtual scene composed of a 3D mesh object, virtual camera, with a rough initial environment lighting map (e.g., constant white ambient light) in Mitsuba2.
We render images for each virtual camera in Mitsuba2 and then minimize
our objective by pushing virtual rendering images similar to real
camera observations with proper regularization. The rendering error then back propagates to update scene parameters for 3D geometry, diffuse and specular reflectance, environment lighting map by auto-diff mechanism, and automatically gradient estimation for non-differentiable parameters. 
Specifically, we start from initial estimated 3D mesh with vertex reflectance, our method optimize diffuse reflectance $\theta_{d}$, and optimize 3D geometry $\theta_{g}$ relying on $\theta_{d}$.
After obtaining $\theta_{d}$ and $\theta_{g}$, our method updates the camera position and pose $\theta_{c}$ and environment light map $\theta_{l}$ by pushing photometric consistency, which allows us further update specular reflection parameter $\theta_{s}$.
We repeat this iterative optimization of inverse rendering and geometric reconstruction until the error converges.
%\paragraph{Photo Realistic View Synthesis}
When the optimized parameters for our real scene are ready, we can synthesize virtual novel and edit current lighting conditions for photo-realistic performance by replacing interested parameters in \eqnref{eqn:image_formation} and running the forward rendering process.


==> related.tex <==
\section{Related Work}\label{sec:related}
Our approach lies at the intersection of several active research areas, namely image based view synthesis, structure from motion (SfM) and multi-view stereo (MVS), volumetric and geometric reconstruction, differentiable rendering. 
In this section, we give a brief review of the above inter-connected topics.

To create photo-realistic novel view, image-based rendering (IBR) ~\cite{szeliski2010computer,chan2007image,zhang2004survey,liu2017new} rely on obtaining high-quality appearances and geometry models or requiring a dense sampling of viewpoint from various angles, novel view can be generated by viewpoint interpolation, 3D geometry and texture projection. Therefore, IBR methods generally require a large number of images from different viewpoints, which becomes a heavy burden for storage and data collection, and basically hard to infer novel view of large viewpoint change or missing information due to occlusion. More details can be referred to \cite{shum2000review}.

Structure from motion (SfM) \cite{LSDSLAMECCV2014, schoenberger2016sfm} estimates 3D scene structure from only a few of viewpoints via feature, image block matching from camera motion or multi-camera system, and then multi-View Stereo (MVS) \cite{schoenberger2016mvs} takes the output of SfM to further compute per-pixel texture matching, depth, surface normal for every pixel in multiple view images. The novel view can be synthesized from a given virtual camera and textured fused point cloud or mesh. Due to lack of reliable feature matching in smooth area of images, 3D model may contain missing hole in mesh or incorrect geometry, therefore, SfM and MVS only preserve main 3D structure of large scale scene but hard to generate photo-realistic detail for novel view.

To synthesize photo realistic novel view, researchers have developed methods that using geometry information, e.g., point clouds~\cite{martin2018lookingood,aliev2019neural,meshry2019neural,dai2020neural},shading and stereo~\cite{maurer2018combining}, and textured meshes~\cite{thies2019deferred,liu2020neural} as input, then novel views are rendered based on the input viewing angle and camera position with proper inpainting or interpolation operation.
However, in the real scene, 3D geometry generally contain geometric error or missing feature points, leads to a failure of geometry reconstruction and texture projection. 

To improve robustness in novel view synthesis, representing 3D scene by implicit function or neural network (e.g., SRN~\cite{sitzmann2019scene}, NeRF~\cite{mildenhall2020nerf}, pixelNeRF\cite{yu2020pixelnerf}, NSVF~\cite{liu2020neural}) has gained popularity recently since it directly represents scene by a implicit volume, and optimizes scene volume via training a self-supervised neural network. Neural representation takes 3D position and camera viewing angle as input, and then outputs interested color, radiance, or voxel density field etc. 
The novel view rendering can be considered as an integral over straight light ray in scene volume. 
Most of scenes (synthetic or real) are not semi-transparent, representing scene as a volume is inaccurate and will ignore the influence of multi-bounce reflection of light, surface reflection (diffuse, specular), camera distance, which are the vital properties to render a photo realistic view.

Differential rendering becomes another promising categories for 3D geometry optimization, texture mapping, high quality novel view rendering. SoftRas~\cite{liu2019soft} propose a differentiable rendering framework that directly render colorized mesh via differentiable functions and back-propagate gradient to mesh vertices, color, silhouette, etc. Li \etal~\cite{li2020inverse} proposed a deep inverse rendering framework for indoor scene shape, spatial-varying light, SVBRDF optimization from single view. \revised{Luan et al. \cite{luan2021unified} proposed a differentiable rendering method for shape and SVBRDF reconstruction by multi view points with initial mesh and designed light source, while our method enables in-the-wild reconstruction.} \cite{Loubet2019Reparameterizing,NimierDavidVicini2019Mitsuba2} proposed a physically-based engine, Mitsuba2, for estimating parameter gradient that based on Monte-Carlo sampling, thus, enables back propagating geometry, and other general scene parameters gradient flow. 
However, directly optimizing scene parameters especially geometry structure of wild scene is still a challenging problem, experiments show the limited toy cases for directly optimization of geometry.

Our proposed method bridges traditional SfM, MVS and differential inverse rendering, first directly infers the rough real scene parameters from 2D images, and automatically build a virtual scene to simulate physical light transmission, finally, optimize scene parameters by a forward rendering and inverse error propagation fashion, enables photo-realistic novel view synthesis that handles large viewpoint change and various camera range. 



%\paragraph{Image-based rendering.}
%To create photo-realistic images, traditional pipelines rely on obtaining high-quality appearances and geometry models, on which global illumination is applied for the rendering process. 
%Directly acquiring 3D models or surface appearance is time-consuming and challenging, especially for complex scenes containing transparent objects, thin structures, or human gestures.  
%Image-based rendering~\cite{szeliski2010computer,chan2007image,zhang2004survey,liu2017new} is then developed to generate novel views by leveraging a sufficient number of input images for view interpolation and vision-based modeling, thus, becomes a heavy burden for storage and data acquisition. More detail reviews can be referred to \cite{shum2000review}.  
%However, IBR methods require a large number of images from different viewpoints, which becomes a heavy burden for storage. 
%
%\paragraph{View synthesis.}
%To synthesize novel view, researchers have developed methods using point clouds~\cite{martin2018lookingood,aliev2019neural,meshry2019neural,dai2020neural}, and textured meshes~\cite{thies2019deferred,liu2020neural} as input, then novel views are rendered based on the input viewing angle and camera position. 
%View synthesis approaches with 3D geometry and texture are proved to work efficiently in applications such as human bodies. 
%Eslami \etal~\cite{eslami2018neural} propose generative query networks to render novel views by learning features embedding 3D scenes and geometrical properties, achieve successful novel view rendering when scene representation and camera extrinsic are given.
%However, since only a simplified feature vector is applied to represent the scene, acquired results are too coarse to be adopted in relatively complicated scenes. 
%To overcome these limitations,
%multiplane images (MPIs)~\cite{flynn2016deepstereo,flynn2019deepview,mildenhall2019local,srinivasan2019pushing} based view synthesis methods have been developed, aiming to improve image quality by learning the 3D structure representations.  
%However, only novel views in limited angles can be generated with MPIs-based techniques. 
%Nguyen-Phuoc \etal~\cite{nguyen2019hologan} propose RenderNet to represent scenes with sparse voxel grids and generate images with CNN decoder. 
%There is a potential issue for view consistency since convolutional kernels are applied in this type of method.  
%Therefore, tight voxel grids~\cite{sitzmann2019deepvoxels,lombardi2019neural} are proposed to improve the quality of generated novel images for view consistency. However, these methods require more storage space. 
%Instead, representing the 3D scene with implicit functions~\cite{mildenhall2020nerf,sitzmann2019scene,wiles2020synsin,liu2020neural,yu2020pixelnerf,tancik2020fourier,lindell2020autoint} has gain popularity recently. For example, Mildenhall~\etal~\cite{mildenhall2020nerf} propose neural radiance fields (NeRF) that represent radiance field by a trained neural network. NeRF achieves good performance for generating spiral style synthetic view (limited view angle), but fail to inference large angle change or zoom in/out. 
%
%\paragraph{Structure from motion, multi-view stereo.}
%Engel \etal~\cite{LSDSLAMECCV2014} propose a direct monocular SLAM algorithm without feature point matching, which allows building large-scale, consistent maps of the environment.
%Schoenberger \etal~\cite{schoenberger2016sfm} propose a systematical framework for incremental Structure-from-Motion pipeline, which improves the robustness and efficiency of correspondence search and incremental reconstruction of the large scene. A Multi-View Stereo (MVS) system \cite{schoenberger2016mvs} is introduced for robust and efficient dense modeling from unstructured image collections and jointly estimate depth and surface normal.
%
%\paragraph{3D reconstruction.}
%3D reconstruction is a vital task in computer vision and graphics.
%Various data representations are used for different applications and tasks, such as light-field-based reconstruction ~\cite{EfficientTOG2016,zhou2018semantic}, tomographic reconstruction~\cite{trifonov2006tomographic,SpaceTOG2018,zang2018super}, polarization ~\cite{PracticalSA2018,BaekTOG2018,ImageSiggraph2020}, shape reconstruction~\cite{gadelha2019shape,wu2018full}, and feature-point based reconstruction~\cite{DensePR2012,PointBasedICCV2013,GlobalICCV2015}. 
%In general, forward rendering and 3D reconstruction can be considered as a pair of forward-backward problems. 
%Forward rendering simulates light traveling and imaging processes, which generates virtual images. 
%By comparing against the real captured images, rendering error can be backward propagated as a gradient for each scene parameter (i.e., 3D geometry, BRDF, reflectance, etc.) by the gradient-based method to optimize the target parameter. \cite{Loubet2019Reparameterizing,NimierDavidVicini2019Mitsuba2} propose decent solutions for estimating gradient based on Monte-Carlo sampling, to name a few.
%
%\paragraph{Differentiable Reconstruction and Rendering}
